WebRelate: Integrating Web Data with Spreadsheets using Examples

Data integration between web sources and relational data is a key challenge faced by data scientists and spreadsheet users. There are two main challenges in programmatically joining web data with relational data. First, most websites do not expose a direct interface to obtain tabular data, so the user needs to formulate a logic to get to different webpages for each input row in the relational table. Second, after reaching the desired webpage, the user needs to write complex scripts to extract the relevant data, which is often conditioned on the input data. Since many data scientists and end-users come from diverse backgrounds, writing such complex regular-expression based logical scripts to perform data integration tasks is unfortunately often beyond their programming expertise. We present WebRelate, a system that allows users to join semi-structured web data with relational data in spreadsheets using input-output examples. WebRelate decomposes the web data integration task into two sub-tasks of i) URL learning and ii) input-dependent web extraction. The first sub-task generates the URLs for the webpages containing the desired data for all rows in the relational table. WebRelate achieves this by learning a string transformation program using a few example URLs. The second sub-task uses examples of desired data to be extracted from the corresponding webpages and learns a program to extract the data for the other rows. We design expressive domain-specific languages for URL generation and web data extraction, and present efficient synthesis algorithms for learning programs in these DSLs from few input-output examples. We evaluate WebRelate on 88 real-world web data integration tasks taken from online help forums and Excel product team, and show that WebRelate can learn the desired programs within few seconds using only 1 example for the majority of the tasks.

==> overview.tex <==
\section{Overview of WebRelate}\seclabel{overview}

An overview of the workflow of the $\sys$ system is shown in \figref{overview}. %As described earlier, $\sys$ decomposes the problem of learning programs to join web data with spreadsheet data into two sub-problems. The first sub-problem learns a program to transform input data to corresponding URL strings. The second sub-problem learns a program  to extract desired data from a web page.
A user starts with some tabular data in a spreadsheet and can provide URL examples in two ways. 1) A user can provide example URLs simply as strings for cases where the URLs can be constructed completely using some transformations on the input data and constant strings. $\sys$ uses the \emph{URL string synthesizer} module to automatically generate the URLs for the other inputs.
 2) A user can provide search query terms, which results in a list of URLs (using a search engine), and then select a URL amongst the results for each example. 
 \sys{} uses the \emph{Search query synthesizer} and the \emph{URL filter synthesizer} to learn the other search queries and URLs.
Given a URL, $\sys$ loads the web page in a neighboring frame, and the user highlights the desired data element to be extracted. The \emph{Data synthesizer} module learns a program  to perform the desired extraction task for the other inputs.
The \emph{URL filter synthesizer} and the \emph{Data synthesizer} modules also use the input spreadsheet data for performing \emph{input-driven ranking} to efficiently learn desired programs from few input-output examples. 

%We now present the DSLs and the corresponding synthesis algorithms for the different synthesis modules in more detail.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/overview.png}
\caption{The workflow of the \sys{} system.}
\figlabel{overview}
\end{figure}
